A Comparative Study of Different Edit Distance-Based Methods for Feature Tracking using Merge Trees on Time-Varying Scalar Fields

Feature tracking in time-varying scalar fields is a fundamental task in scientific computing. Topological descriptors, which summarize important features of data, have proved to be viable tools to facilitate this task. The merge tree is a topological descriptor that captures the connectivity behaviors of the sub- or superlevel sets of a scalar field. Edit distances between merge trees play a vital role in effective temporal data tracking. Existing methods to compute them fall into two main classes, namely whether they are dependent or independent of the branch decomposition. These two classes represent the most prominent approaches for producing tracking results. In this paper, we compare four different merge tree edit distance-based methods for feature tracking. We demonstrate that these methods yield distinct results with both analytical and real-world data sets. Furthermore, we investigate how these results vary and identify the factors that influence them. Our experiments reveal significant differences in tracked features over time, even among those produced by techniques within the same category.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = MergeTreeTrackingCompr.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = Literature.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> supp_Bousinesq2D.tex <==
\subsection*{Results using Boussinesq2D}
The results of the experiments using \dataset{Boussinesq2D}
are shown from \Cref{fig-Boussinesq2DAllNodes}
to \Cref{fig-Boussinesq2DSimilarities}.

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Boussinesq2D/all_node_pairs_distribution.pdf}
\caption{
    Number of tracked nodes (colored and labeled) 
    relative to the total nodes of merge trees (light blue bars)
    for \dataset{Boussinesq2D}.
}
\label{fig-Boussinesq2DAllNodes}
\end{figure}

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Boussinesq2D/critical_types_violin.pdf}
\caption{
    Distributions of tracked nodes 
    over the chosen time steps of \dataset{Boussinesq2D},  
    divided by types:
    saddle (yellow) and minima (blue).
}
\label{fig-Boussinesq2DViolin}
\end{figure}


% Length histogram
\begin{figure}%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Boussinesq2D/W_tracking_length_histograms.pdf}
\caption{$d_w$.}%
\label{fig-LengthHistogramBoussinesq2DW}%
\end{subfigure}
%
\hfill%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Boussinesq2D/E_tracking_length_histograms.pdf}%
\caption{$d_e$.}%
\label{fig-LengthHistogramBoussinesq2DE}%
\end{subfigure}%
%
\\%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Boussinesq2D/B_tracking_length_histograms.pdf}%
\caption{$d_b$.}%
\label{fig-LengthHistogramBoussinesq2DB}%
\end{subfigure}%
%
\hfill%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Boussinesq2D/P_tracking_length_histograms.pdf}%
\caption{$d_p$.}%
\label{fig-LengthHistogramBoussinesq2DP}%
\end{subfigure}%
%
\caption{Histograms of the length of the tracking paths 
    using the last $1000$ time steps
    of \dataset{Boussinesq2D}.}%
\label{fig-LengthHisgoramBoussinesq2D}%
\end{figure}

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Boussinesq2D/similarity.pdf}
\caption{
    Pairwise differences between the methods on the columns
    in relation to the methods on the rows
    for \dataset{Boussinesq2D}.
}
\label{fig-Boussinesq2DSimilarities}
\end{figure}

==> supp_Cylinder2D.tex <==
\subsection*{Extra results with Cylinder2D data set}
More results of the experiments using \dataset{Cylinder2D}
are shown in \Cref{fig-Cylinder2DAllNodesLong}
through \Cref{fig-LengthHisgoramCylinder2DLong}.


\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Cylinder2D/all_node_pairs_distribution.pdf}
\caption{
    Number of tracked nodes (colored and labeled) 
    relative to the total nodes of merge trees (light blue bars)
    for \dataset{Cylinder2D}.
}
\label{fig-Cylinder2DAllNodesLong}
\end{figure}


% Length histogram
\begin{figure}%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Cylinder2D/W_tracking_length_histograms.pdf}
\caption{$d_w$.}%
\label{fig-LengthHistogramCylinder2DWLong}%
\end{subfigure}
%
\hfill%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Cylinder2D/E_tracking_length_histograms.pdf}%
\caption{$d_e$.}%`'
\label{fig-LengthHistogramCylinder2DELong}%
\end{subfigure}%
%
\\%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Cylinder2D/B_tracking_length_histograms.pdf}%
\caption{$d_b$.}%
\label{fig-LengthHistogramCylinder2DBLong}%
\end{subfigure}%
%
\hfill%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Cylinder2D/P_tracking_length_histograms.pdf}%
\caption{$d_p$.}%
\label{fig-LengthHistogramCylinder2DPLong}%
\end{subfigure}%
%
\caption{Histograms of the length of the tracking paths
    of \dataset{Cylinder2D}.}%
\label{fig-LengthHisgoramCylinder2DLong}%
\end{figure}


==> supp_Cylinder3D.tex <==
\subsection*{Results using Cylinder3D}
The results of the experiments using \dataset{Cylinder3D}
are shown from \Cref{fig-Cylinder3DAllNodes}
to \Cref{fig-Cylinder3DSimilarities}.

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Cylinder3D/all_node_pairs_distribution.pdf}
\caption{
    Number of tracked nodes (colored and labeled) 
    relative to the total nodes of merge trees (light blue bars)
    for \dataset{Cylinder3D}.
}
\label{fig-Cylinder3DAllNodes}
\end{figure}

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Cylinder3D/critical_types_violin.pdf}
\caption{
    Distributions of tracked nodes 
    of \dataset{Cylinder3D},  
    divided by types:
    saddle (yellow) and minima (blue).
}
\label{fig-Cylinder3DViolin}
\end{figure}


% Length histogram
\begin{figure}%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Cylinder3D/W_tracking_length_histograms.pdf}
\caption{$d_w$.}%
\label{fig-LengthHistogramCylinder3DW}%
\end{subfigure}
%
\hfill%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Cylinder3D/E_tracking_length_histograms.pdf}%
\caption{$d_e$.}%
\label{fig-LengthHistogramCylinder3DE}%
\end{subfigure}%
%
\\%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Cylinder3D/B_tracking_length_histograms.pdf}%
\caption{$d_b$.}%
\label{fig-LengthHistogramCylinder3DB}%
\end{subfigure}%
%
\hfill%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Cylinder3D/P_tracking_length_histograms.pdf}%
\caption{$d_p$.}%
\label{fig-LengthHistogramCylinder3DP}%
\end{subfigure}%
%
\caption{Histograms of the length of the tracking paths 
    of \dataset{Cylinder3D}.}%
\label{fig-LengthHisgoramCylinder3D}%
\end{figure}

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Cylinder3D/similarity.pdf}
\caption{
    Pairwise differences between the methods on the columns
    in relation to the methods on the rows
    for \dataset{Cylinder3D}.
}
\label{fig-Cylinder3DSimilarities}
\end{figure}

==> supp_IonizationFront.tex <==
\subsection*{Results using IonizationFront2D}
The results of the experiments using \dataset{IonizationFront2D}
are shown from \Cref{fig-IonizationFront2DAllNodes}
to \Cref{fig-IonizationFront2DSimilarities}.

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/IonizationFront2D/all_node_pairs_distribution_short.pdf}
\caption{
    Number of tracked nodes (colored and labeled) 
    relative to the total nodes of merge trees (light blue bars)
    for \dataset{IonizationFront2D}.
}
\label{fig-IonizationFront2DAllNodes}
\end{figure}

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/IonizationFront2D/critical_types_violin.pdf}
\caption{
    Distributions of tracked nodes 
    over the chosen time steps of \dataset{IonizationFront2D},  
    divided by types:
    saddle (yellow) and maxima (red).
}
\label{fig-IonizationFront2DViolin}
\end{figure}


% Length histogram
\begin{figure}%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/IonizationFront2D/W_tracking_length_histograms_short.pdf}
\caption{$d_w$.}%
\label{fig-LengthHistogramIonizationFront2DW}%
\end{subfigure}
%
\hfill%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/IonizationFront2D/E_tracking_length_histograms_short.pdf}%
\caption{$d_e$.}%
\label{fig-LengthHistogramIonizationFront2DE}%
\end{subfigure}%
%
\\%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/IonizationFront2D/B_tracking_length_histograms_short.pdf}%
\caption{$d_b$.}%
\label{fig-LengthHistogramIonizationFront2DB}%
\end{subfigure}%
%
\hfill%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/IonizationFront2D/P_tracking_length_histograms_short.pdf}%
\caption{$d_p$.}%
\label{fig-LengthHistogramIonizationFront2DP}%
\end{subfigure}%
%
\caption{Histograms of the length of the tracking paths of the first $100$ time steps 
    of \dataset{IonizationFront2D}.}%
\label{fig-LengthHisgoramIonizationFront2D}%
\end{figure}

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/IonizationFront2D/similarity.pdf}
\caption{
    Pairwise differences between the methods on the columns
    in relation to the methods on the rows
    for \dataset{IonizationFront2D}.
}
\label{fig-IonizationFront2DSimilarities}
\end{figure}

==> supp_Storms2D.tex <==
\subsection*{Results using Storms2D}
The results of the experiments using \dataset{Storms2D}
are shown from \Cref{fig-Storms2DAllNodes}
to \Cref{fig-Storms2DSimilarities}.

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Storms2D/all_node_pairs_distribution.pdf}
\caption{
    Number of tracked nodes (colored and labeled) 
    relative to the total nodes of merge trees (light blue bars)
    for \dataset{Storms2D}.
}
\label{fig-Storms2DAllNodes}
\end{figure}

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Storms2D/critical_types_violin.pdf}
\caption{
    Distributions of tracked nodes 
    of \dataset{Storms2D},  
    divided by types:
    saddle (yellow) and minima (blue).
}
\label{fig-Storms2DViolin}
\end{figure}


% Length histogram
\begin{figure}%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Storms2D/W_tracking_length_histograms.pdf}
\caption{$d_w$.}%
\label{fig-LengthHistogramStorms2DW}%
\end{subfigure}
%
\hfill%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Storms2D/E_tracking_length_histograms.pdf}%
\caption{$d_e$.}%
\label{fig-LengthHistogramStorms2DE}%
\end{subfigure}%
%
\\%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Storms2D/B_tracking_length_histograms.pdf}%
\caption{$d_b$.}%
\label{fig-LengthHistogramStorms2DB}%
\end{subfigure}%
%
\hfill%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Storms2D/P_tracking_length_histograms.pdf}%
\caption{$d_p$.}%
\label{fig-LengthHistogramStorms2DP}%
\end{subfigure}%
%
\caption{Histograms of the length of the tracking paths 
    of \dataset{Storms2D}.}%
\label{fig-LengthHisgoramStorms2D}%
\end{figure}

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Storms2D/similarity.pdf}
\caption{
    Pairwise differences between the methods on the columns
    in relation to the methods on the rows
    for \dataset{Storms2D}.
}
\label{fig-Storms2DSimilarities}
\end{figure}

==> supp_Tangaroa.tex <==
\subsection*{Results with Tangaroa data set}
The results of the experiments using \dataset{Tangaroa3D}
are shown in \Cref{fig-Tangaroa3DAllNodes}
through \Cref{fig-Tangaroa3DSimilarities}.

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Tangaroa3D/all_node_pairs_distribution_short.pdf}
\caption{
    Number of tracked nodes (colored and labeled) 
    relative to the total nodes of merge trees (light blue bars)
    for \dataset{Tangaroa3D}.
}
\label{fig-Tangaroa3DAllNodes}
\end{figure}

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Tangaroa3D/critical_types_violin.pdf}
\caption{
    Distributions of tracked nodes 
    \dataset{Tangaroa3D},  
    divided by types:
    saddle (yellow) and maxima (red).
}
\label{fig-Tangaroa3DViolin}
\end{figure}


% Length histogram
\begin{figure}%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Tangaroa3D/W_tracking_length_histograms_short.pdf}
\caption{$d_w$.}%
\label{fig-LengthHistogramTangaroa3DW}%
\end{subfigure}
%
\hfill%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Tangaroa3D/E_tracking_length_histograms_short.pdf}%
\caption{$d_e$.}%
\label{fig-LengthHistogramTangaroa3DE}%
\end{subfigure}%
%
\\%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Tangaroa3D/B_tracking_length_histograms_short.pdf}%
\caption{$d_b$.}%
\label{fig-LengthHistogramTangaroa3DB}%
\end{subfigure}%
%
\hfill%
%
\begin{subfigure}[t]{\ltwopicwidth}%
\includegraphics[width=\ltwopicwidth]{supp_img/Tangaroa3D/P_tracking_length_histograms_short.pdf}%
\caption{$d_p$.}%
\label{fig-LengthHistogramTangaroa3DP}%
\end{subfigure}%
%
\caption{Histograms of the length of the tracking paths
    of \dataset{Tangaroa3D}.}%
\label{fig-LengthHisgoramTangaroa3D}%
\end{figure}

\begin{figure}
%
\centering
%
\includegraphics[width=0.8\linewidth]{supp_img/Tangaroa3D/similarity.pdf}
\caption{
    Pairwise differences between the methods on the columns
    in relation to the methods on the rows
    for \dataset{Tangaroa3D}.
}
\label{fig-Tangaroa3DSimilarities}
\end{figure}

==> supp_extraData.tex <==
\section*{Extra Results on Real-World Data Set}
We introduce information on the data sets used in this section,
followed by the results for each of them. 

\dataset{IonizationFront2D} is a simulated 2D scalar field 
from 2008 SciVis Contest \cite{whalen2008competition},  
The results 
capture the formation of the first stars in the universe 
through density variations of the so-called ionization front.
We use the first $100$ time steps for our experiment.
The split trees can be used to map the regions with similar density
as the shadow instability progresses.

\dataset{Storms2D} depicts a one-hourly mean sea level pressure 
over the month of December 1999. This data set is available to download at 
\cite{ERA5data}. Similar to K\"opp and Weinkauf \cite{koepp22},
the mean over eight days is computed and a light Gaussian smoothing is applied.
This process creates a time-dependent 2D scalar field with 743 time steps.
The structural changes in join trees over time 
provide insight into the formation and evolution of storms.

\dataset{Boussinesq2D} is a simulation of a flow generated 
by a heated cylinder \cite{Guenther17} over $2001$ time steps
using Gerris flow solver \cite{germer11a}.
It is a time-dependent vector field and 
contains numerous small vortices rotating around each other.
Using the last $1000$ time steps, we compute and 
track the evolution of join trees of the velocity magnitude,
as their nodes associate with the vortex centers.

\dataset{Cylinder3D} originates from a simulation of 3D turbulent flow 
around a half-cylinder. \cite{BaezaRojo19SciVisa} with
the Reynolds number of $640$. 
It contains $151$ time steps.
The split trees are employed to track the temporal evolution of the 
local maxima and saddle points of the velocity magnitude.

\dataset{Tangaroa3D} captures the 3D flow around a research vessel Tangaroa
over $200$ time steps \cite{PopinetEtAl2004_Tangaroa}.
Similar to Cylinder3D, we also compute the magnitude of the velocity
to obtain a scalar field for each time step.
We also track the evolution of split trees of 
resulted from the velocity magnitude.



The three data sets \dataset{Boussinesq2D}, \dataset{Cylinder3D}, and \dataset{Tangaroa3D}
can be found at the
\href{https://cgl.ethz.ch/research/visualization/data.php}{Computer Graphics Laboratory}.
The simplification thresholds for the data sets are:
\dataset{IonizationFront2D} at $5\%$,
\dataset{Storms2D} at $1\%$,
\dataset{Boussinesq2D} at $2\%$,
both \dataset{Cylinder3D} and \dataset{Tangaroa3D} at $8\%$.
We also provide results for with more time steps of \dataset{Cylinder2D}.


\input{supp_IonizationFront}

\input{supp_Storms2D}

\input{supp_Bousinesq2D}

\input{supp_Cylinder3D}

\input{supp_Tangaroa}

\input{supp_Cylinder2D}

==> supp_stableNoise.tex <==
\section*{Stability with respect to Noise}
In the section, we show the results of the stability score 
with $\epsilon_\text{max} = 5\%$. 
The results can be seen 
in \Cref{fig-stab10}, \Cref{fig-stab15}, and \Cref{fig-stab20}.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{StableNoise/leaves_stability_quantile_0.1}
    \caption{The tracking stability of the extrema of the for methods 
    if we stop at $\epsilon_\text{max}=10\%$. 
    }
    \label{fig-stab10}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{StableNoise/leaves_stability_quantile_0.15}
    \caption{The tracking stability of the extrema of the for methods 
    if we stop at $\epsilon_\text{max}=15\%$.}
    \label{fig-stab15}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{StableNoise/leaves_stability_quantile_0.2}
    \caption{The tracking stability of the extrema of the for methods 
    if we stop at $\epsilon_\text{max}=20\%$.}
    \label{fig-stab20}
\end{figure}
